A matterless double slit

Double-slits provide incoming photons with a choice. Those that survive the passage have chosen from two possible paths which interfere to distribute them in a wave-like manner. Such wave-particle duality continues to be challenged and investigated in a broad range of disciplines with electrons, neutrons, helium atoms, C60 fullerenes, Bose-Einstein condensates and biological molecules. All variants have hitherto involved material constituents. We present a matterless double-slit scenario in which photons generated from virtual electron-positron pair annihilation in head-on collisions of a probe laser field with two ultra-intense laser beams form a double-slit interference pattern. Such electromagnetic fields are predicted to induce material-like behaviour in the vacuum, supporting elastic scattering between photons. Our double-slit scenario presents on the one hand a realisable method to observe photon-photon scattering, and demonstrates on the other, the possibility of both controlling light with light and non-locally investigating features of the quantum vacuum's structure.

==> PaxHeader/DS_nature_photonics_sendable_full.tex <==
17 gid=683622706
18 uid=1425403446
20 ctime=1359488505
20 atime=1359488505
24 SCHILY.dev=234881026
23 SCHILY.ino=16227245
18 SCHILY.nlink=1

